Astrophysics and cosmology with a decihertz gravitational-wave detector: TianGO

We present the astrophysical science case for a space-based, decihertz gravitational-wave (GW) detector. We particularly highlight an ability to infer a source's sky location, both when combined with a network of ground-based detectors to form a long triangulation baseline, and by itself for the early warning of merger events. Such an accurate location measurement is the key for using GW signals as standard sirens for constraining the Hubble constant. This kind of detector also opens up the possibility to test type Ia supernovae progenitor hypotheses by constraining the merger rates of white dwarf binaries with both super- and sub-Chandrasekhar masses separately. We will discuss other scientific outcomes that can be delivered, including the constraint of structure formation in the early Universe, the search for intermediate-mass black holes, the precise determination of black hole spins, the probe of binary systems' orbital eccentricity evolution, and the detection of tertiary masses around merging binaries.

==> LocalizationTableArcsec.tex <==
HLV & $1.0\times 10^{5}$ & $5.3\times 10^{5}$ & $1.4\times 10^{6}$ & $7.0\times 10^{6}$ \\
HLVKA & $2.6\times 10^{4}$ & $7.3\times 10^{4}$ & $3.1\times 4.0^{4}$ & $1.1\times 10^{5}$ \\
T & $454$ & $700$ & $5.7\times 10^{4}$ & $1.4\times 10^{5}$ \\
HLVKA + L2 T & $207$ & $376$ & $7000$ & $1.9\times 10^{4}$ \\
HLVKA + $5^\circ$ T & $74$ & $168$ & $855$ & $2460$ \\
HLVKA + $20^\circ$ T & $17$ & $45$ & $207$ & $674$ \\


==> LocalizationTableDot.tex <==
HLV & $7.9\cdot 10^{-3}$ & $4.1\cdot 10^{-2}$ & $1.1\cdot 10^{-2}$ & $5.4\cdot 10^{-2}$ \\
HLVKA & $2.0\cdot 10^{-3}$ & $5.6\cdot 10^{-3}$ & $3.1\cdot 10^{-3}$ & $8.5\cdot 10^{-3}$ \\
T & $3.5\cdot 10^{-5}$ & $5.4\cdot 10^{-5}$ & $4.4\cdot 10^{-3}$ & $1.1\cdot 10^{-2}$ \\
HLVKA + L2 T & $1.6\cdot 10^{-5}$ & $2.9\cdot 10^{-5}$ & $5.4\cdot 10^{-4}$ & $1.5\cdot 10^{-3}$ \\
HLVKA + $5^\circ$ T & $5.7\cdot 10^{-6}$ & $1.3\cdot 10^{-5}$ & $6.6\cdot 10^{-5}$ & $1.9\cdot 10^{-4}$ \\
HLVKA + $20^\circ$ T & $1.3\cdot 10^{-6}$ & $3.5\cdot 10^{-6}$ & $1.6\cdot 10^{-5}$ & $5.2\cdot 10^{-5}$ \\

